Implementing QZMAC (a Decentralized Delay Optimal MAC) over 6TiSCH under the Contiki OS in an IEEE 802.15.4 Network

Motivated by the emerging delay-sensitive applications of the Internet of Things (IoT), there has been a resurgence of interest in developing medium access control (MAC) protocols in a time-slotted framework. The resource-constrained, ad-hoc nature of wireless networks typical of the IoT also forces the amount of control information exchanged across the network -- required to make scheduling decisions -- to a minimum. In a previous article we proposed a protocol called QZMAC that (i) provides provably low mean delay, (ii) has distributed control (i.e., there is no central scheduler), and (iii) does not require explicit exchange of state information or control signals. In the present article, we implement and demonstrate the performance of QZMAC on a test bed consisting of CC2420 based Crossbow telosB motes, running the 6TiSCH communication stack on the Contiki operating system over the 2.4GHz ISM band. QZMAC achieves its near-optimal delay performance using a clever combination of polling and contention modes. We demonstrate the polling and the contention modes of QZMAC separately. We use an Adaptive Synchronization Technique in our implementation which we also demonstrate. Our network shows good delay performance even in the presence of heavy interference from ambient WiFi networks.

==> figures/figure_embedding_queueing_and_arrival_processes.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\resizebox{9.00cm}{5.0cm}{
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,392); %set diagram left start at 0, and has height of 392

%Straight Lines [id:da1949052064879535] 
\draw [line width=1.5]    (89.3,167.98) -- (89.3,263.38) ;
%Straight Lines [id:da6104147472630517] 
\draw [line width=1.5]    (341.3,168.98) -- (341.3,262.38) ;
%Curve Lines [id:da4775364940921927] 
\draw [color={rgb, 255:red, 15; green, 64; blue, 230 }  ,draw opacity=1 ][line width=1.5]    (119.3,141.98) .. controls (73.99,163.65) and (139.29,168.82) .. (92.52,189.04) ;
\draw [shift={(90.3,189.98)}, rotate = 337.62] [color={rgb, 255:red, 15; green, 64; blue, 230 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Curve Lines [id:da2984703398201145] 
\draw [color={rgb, 255:red, 15; green, 64; blue, 230 }  ,draw opacity=1 ][line width=1.5]    (371.3,151.98) .. controls (325.99,173.65) and (391.29,178.82) .. (344.52,199.04) ;
\draw [shift={(342.3,199.98)}, rotate = 337.62] [color={rgb, 255:red, 15; green, 64; blue, 230 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da1297417084088166] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (341.3,94.38) -- (341.3,162.98) ;
\draw [shift={(341.3,165.98)}, rotate = 270] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da7792126148642344] 
\draw [color={rgb, 255:red, 15; green, 64; blue, 230 }  ,draw opacity=1 ][line width=1.5]    (93.3,230.68) -- (183.3,230.68) ;
\draw [shift={(89.3,230.68)}, rotate = 0] [fill={rgb, 255:red, 15; green, 64; blue, 230 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da886504007318129] 
\draw [color={rgb, 255:red, 15; green, 64; blue, 230 }  ,draw opacity=1 ][line width=1.5]    (337.3,231.68) -- (237.3,231.68) ;
\draw [shift={(341.3,231.68)}, rotate = 180] [fill={rgb, 255:red, 15; green, 64; blue, 230 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Curve Lines [id:da2386457917406799] 
\draw [color={rgb, 255:red, 90; green, 156; blue, 18 }  ,draw opacity=1 ][line width=1.5]    (330.3,262.98) .. controls (284.99,284.65) and (350.29,289.82) .. (303.52,310.04) ;
\draw [shift={(301.3,310.98)}, rotate = 337.62] [color={rgb, 255:red, 90; green, 156; blue, 18 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da39519527174802227] 
\draw [line width=2.25]    (39.3,262.98) -- (621.3,262.98) ;

% Text Node
\draw (120,121.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{1.12em}{1.34em}\selectfont,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$Q_{j}( t)$};
% Text Node
\draw (361,129.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{1em}{1.2em}\selectfont,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$Q_{j}( t+1) \ =\ ( Q_{j}( t) -D_{j}( t))^{+} \ +\ A_{j}( t+1)$};
% Text Node
\draw (311,68.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{1.12em}{1.34em}\selectfont,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$A_{j}( t+1)$};
% Text Node
\draw (188,221) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{1.13em}{1.36em}\selectfont] [align=left] {Slot $\displaystyle t$};
% Text Node
\draw (260,314.4) node [anchor=north west][inner sep=0.75pt]  [font=\fontsize{1.12em}{1.34em}\selectfont]  {$D_{j}( t)$};


\end{tikzpicture}
}

==> figures/geo-d-x-1-alarm-traffic.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,671); %set diagram left start at 0, and has height of 671

%Straight Lines [id:da22031459393974595] 
\draw    (169.51,122.96) -- (325.5,122.96) ;
%Straight Lines [id:da809027084309204] 
\draw    (326.5,121.96) -- (326.5,181.91) ;
%Straight Lines [id:da1236798655371556] 
\draw    (171.19,181.91) -- (327.18,181.91) ;
%Rounded Rect [id:dp5233083168331873] 
\draw   (313.13,125.68) .. controls (317.62,125.64) and (321.29,129.25) .. (321.32,133.74) -- (321.59,168.96) .. controls (321.63,173.46) and (318.01,177.12) .. (313.52,177.16) -- (289.13,177.36) .. controls (284.64,177.39) and (280.97,173.78) .. (280.94,169.29) -- (280.67,134.07) .. controls (280.63,129.58) and (284.24,125.91) .. (288.74,125.87) -- cycle ;
%Curve Lines [id:da7819448564534215] 
\draw    (114.05,102.41) .. controls (154.97,103.16) and (135.44,135.58) .. (168.17,138) ;
\draw [shift={(169.7,138.09)}, rotate = 182.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da10246095311611136] 
\draw    (110.79,204.48) .. controls (151.72,205.22) and (132.91,172.41) .. (165.66,172.87) ;
\draw [shift={(167.19,172.91)}, rotate = 182.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8696881549024784] 
\draw    (113.31,153.57) -- (163.98,153.57) ;
\draw [shift={(165.98,153.57)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6387613299825519] 
\draw    (342,149.42) -- (450.31,217.36) ;
\draw [shift={(452,218.42)}, rotate = 212.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp4328260514515727] 
\draw   (453.34,236.98) .. controls (453.34,226.55) and (461.64,218.09) .. (471.88,218.09) .. controls (482.13,218.09) and (490.43,226.55) .. (490.43,236.98) .. controls (490.43,247.41) and (482.13,255.87) .. (471.88,255.87) .. controls (461.64,255.87) and (453.34,247.41) .. (453.34,236.98) -- cycle ;
%Shape: Ellipse [id:dp6011641419862526] 
\draw   (86.07,171.01) .. controls (86.05,169.52) and (87.22,168.31) .. (88.69,168.31) .. controls (90.15,168.31) and (91.34,169.52) .. (91.36,171.01) .. controls (91.37,172.49) and (90.2,173.7) .. (88.74,173.7) .. controls (87.28,173.7) and (86.08,172.49) .. (86.07,171.01) -- cycle ;
%Shape: Ellipse [id:dp9160539049965806] 
\draw   (86.07,183.09) .. controls (86.05,181.61) and (87.22,180.4) .. (88.69,180.4) .. controls (90.15,180.4) and (91.34,181.61) .. (91.36,183.09) .. controls (91.37,184.58) and (90.2,185.79) .. (88.74,185.79) .. controls (87.28,185.79) and (86.08,184.58) .. (86.07,183.09) -- cycle ;
%Shape: Ellipse [id:dp2548490997188926] 
\draw   (86.07,194.43) .. controls (86.05,192.94) and (87.22,191.73) .. (88.69,191.73) .. controls (90.15,191.73) and (91.34,192.94) .. (91.36,194.43) .. controls (91.37,195.92) and (90.2,197.12) .. (88.74,197.12) .. controls (87.28,197.12) and (86.08,195.92) .. (86.07,194.43) -- cycle ;
%Straight Lines [id:da4829040878418136] 
\draw    (173.51,303.96) -- (329.5,303.96) ;
%Straight Lines [id:da16385700890178212] 
\draw    (329.5,303.96) -- (329.5,381.29) ;
%Straight Lines [id:da26982391974540065] 
\draw    (173.51,381.29) -- (329.5,381.29) ;
%Rounded Rect [id:dp6275580880577942] 
\draw   (316.5,307.68) .. controls (321.34,307.64) and (325.29,311.53) .. (325.33,316.36) -- (325.72,368.4) .. controls (325.76,373.24) and (321.87,377.19) .. (317.04,377.23) -- (290.77,377.44) .. controls (285.94,377.48) and (281.99,373.59) .. (281.95,368.76) -- (281.55,316.72) .. controls (281.52,311.88) and (285.41,307.93) .. (290.24,307.89) -- cycle ;
%Rounded Rect [id:dp876197579306828] 
\draw   (268.28,307.28) .. controls (273.11,307.24) and (277.06,311.12) .. (277.1,315.96) -- (277.5,368) .. controls (277.54,372.83) and (273.65,376.78) .. (268.81,376.82) -- (242.55,377.03) .. controls (237.71,377.07) and (233.76,373.18) .. (233.73,368.35) -- (233.33,316.31) .. controls (233.29,311.48) and (237.18,307.53) .. (242.01,307.49) -- cycle ;
%Rounded Rect [id:dp9002066434368925] 
\draw   (219.31,307.63) .. controls (224.14,307.59) and (228.09,311.47) .. (228.13,316.31) -- (228.53,368.35) .. controls (228.57,373.18) and (224.68,377.13) .. (219.84,377.17) -- (193.58,377.38) .. controls (188.75,377.42) and (184.8,373.54) .. (184.76,368.7) -- (184.36,316.66) .. controls (184.32,311.83) and (188.21,307.88) .. (193.05,307.84) -- cycle ;
%Curve Lines [id:da9990295143760162] 
\draw    (118.05,284.41) .. controls (158.97,285.16) and (139.44,317.58) .. (172.17,320) ;
\draw [shift={(173.7,320.09)}, rotate = 182.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da956697574514191] 
\draw    (118.79,395.48) .. controls (159.72,396.22) and (140.91,363.41) .. (173.66,363.87) ;
\draw [shift={(175.19,363.91)}, rotate = 182.48] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9546732899311114] 
\draw    (117.31,337.57) -- (167.98,337.57) ;
\draw [shift={(169.98,337.57)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp3268470988936958] 
\draw   (99.07,355.01) .. controls (99.05,353.52) and (100.22,352.31) .. (101.69,352.31) .. controls (103.15,352.31) and (104.34,353.52) .. (104.36,355.01) .. controls (104.37,356.49) and (103.2,357.7) .. (101.74,357.7) .. controls (100.28,357.7) and (99.08,356.49) .. (99.07,355.01) -- cycle ;
%Shape: Ellipse [id:dp7512359084056817] 
\draw   (99.07,367.09) .. controls (99.05,365.61) and (100.22,364.4) .. (101.69,364.4) .. controls (103.15,364.4) and (104.34,365.61) .. (104.36,367.09) .. controls (104.37,368.58) and (103.2,369.79) .. (101.74,369.79) .. controls (100.28,369.79) and (99.08,368.58) .. (99.07,367.09) -- cycle ;
%Shape: Ellipse [id:dp9523132295402834] 
\draw   (99.07,378.43) .. controls (99.05,376.94) and (100.22,375.73) .. (101.69,375.73) .. controls (103.15,375.73) and (104.34,376.94) .. (104.36,378.43) .. controls (104.37,379.92) and (103.2,381.12) .. (101.74,381.12) .. controls (100.28,381.12) and (99.08,379.92) .. (99.07,378.43) -- cycle ;
%Rounded Rect [id:dp11998227575694465] 
\draw   (267.47,126) .. controls (271.96,125.97) and (275.63,129.58) .. (275.67,134.07) -- (275.94,169.29) .. controls (275.97,173.78) and (272.36,177.45) .. (267.87,177.49) -- (243.48,177.68) .. controls (238.99,177.72) and (235.32,174.11) .. (235.28,169.62) -- (235.01,134.39) .. controls (234.98,129.9) and (238.59,126.23) .. (243.08,126.2) -- cycle ;
%Rounded Rect [id:dp7891992415493496] 
\draw   (219.82,126.33) .. controls (224.31,126.29) and (227.98,129.9) .. (228.01,134.39) -- (228.28,169.62) .. controls (228.32,174.11) and (224.71,177.78) .. (220.22,177.81) -- (195.82,178.01) .. controls (191.33,178.05) and (187.67,174.43) .. (187.63,169.94) -- (187.36,134.72) .. controls (187.33,130.23) and (190.94,126.56) .. (195.43,126.52) -- cycle ;
%Straight Lines [id:da7843216351222155] 
\draw    (344,343.42) -- (449.46,255.7) ;
\draw [shift={(451,254.42)}, rotate = 500.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da27294524730981307] 
\draw    (385,143.42) .. controls (361.12,159.34) and (332.29,312.88) .. (388.15,350.86) ;
\draw [shift={(389,351.42)}, rotate = 212.99] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1688864951173159] 
\draw    (490.43,236.98) -- (541.11,236.98) ;
\draw [shift={(543.11,236.98)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (60.68,141.6) node [anchor=north west][inner sep=0.75pt]    {$A^{( a)}_{2}( t)$};
% Text Node
\draw (63.19,203.51) node [anchor=north west][inner sep=0.75pt]    {$A_{N}( t)$};
% Text Node
\draw (62.45,92.71) node [anchor=north west][inner sep=0.75pt]    {$A^{( a)}_{1}( t)$};
% Text Node
\draw (74.68,326.6) node [anchor=north west][inner sep=0.75pt]    {$A_{2}( t)$};
% Text Node
\draw (74.19,384.51) node [anchor=north west][inner sep=0.75pt]    {$A_{N}( t)$};
% Text Node
\draw (73.45,275.71) node [anchor=north west][inner sep=0.75pt]    {$A_{1}( t)$};
% Text Node
\draw (200,97.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {\small Alarm Packets};
% Text Node
\draw (213,279.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {\small Data Packets};
% Text Node
\draw (401,160.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {\small Higher Priority};
% Text Node
\draw (435.5,306.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {\small Lower Priority};
% Text Node
\draw (380,320.42) node [anchor=north west][inner sep=0.75pt]   [align=left] {\small{(Serve only if alarm queue is empty)}};


\end{tikzpicture}

==> figures/geo-x-d-1queue.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.5pt,y=0.5pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da21091821527862487] 
\draw[very thick,black]    (181,111) -- (391.26,111) ;
%Straight Lines [id:da8923248760987523] 
\draw[very thick,black]    (391.26,111) -- (391.26,213.35) ;
%Straight Lines [id:da8966019854695426] 
\draw[very thick,black]    (181,213.35) -- (391.26,213.35) ;
%Rounded Rect [id:dp9740766065249149] 
\filldraw[very thick, fill=blue!60!white!40, draw=black]  (373.74,115.93) .. controls (380.26,115.88) and (385.58,121.12) .. (385.64,127.64) -- (386.17,196.09) .. controls (386.22,202.6) and (380.98,207.93) .. (374.47,207.98) -- (339.06,208.26) .. controls (332.55,208.31) and (327.22,203.07) .. (327.17,196.55) -- (326.63,128.1) .. controls (326.58,121.58) and (331.82,116.26) .. (338.34,116.21) -- cycle ;
%Rounded Rect [id:dp058046820249539444] 
\filldraw[very thick, fill=blue!60!white!40, draw=black] (308.74,115.39) .. controls (315.26,115.34) and (320.58,120.58) .. (320.63,127.1) -- (321.17,195.55) .. controls (321.22,202.07) and (315.98,207.39) .. (309.46,207.44) -- (274.06,207.72) .. controls (267.54,207.77) and (262.22,202.53) .. (262.16,196.01) -- (261.63,127.57) .. controls (261.58,121.05) and (266.82,115.72) .. (273.34,115.67) -- cycle ;
%Rounded Rect [id:dp2739897468562962] 
\filldraw[very thick, fill=blue!60!white!40, draw=black]  (242.73,115.86) .. controls (249.25,115.81) and (254.58,121.05) .. (254.63,127.57) -- (255.16,196.01) .. controls (255.22,202.53) and (249.97,207.86) .. (243.46,207.91) -- (208.05,208.19) .. controls (201.54,208.24) and (196.21,203) .. (196.16,196.48) -- (195.62,128.03) .. controls (195.57,121.51) and (200.81,116.19) .. (207.33,116.14) -- cycle ;
%Curve Lines [id:da09849830586458941] 
\draw   (106.25,85.13) .. controls (161.69,86.12) and (134.81,129.47) .. (179.87,132.28) ;
\draw [shift={(181.26,132.35)}, rotate = 182.44] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da3026930486770598] 
\draw    (107.25,232.13) .. controls (162.69,233.12) and (136.79,189.24) .. (181.87,190.31) ;
\draw [shift={(183.26,190.35)}, rotate = 182.44] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4007844786240109] 
\draw    (105.25,158.13) -- (174.25,158.13) ;
\draw [shift={(176.25,158.13)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3706975149666767] 
% \draw[thick,black,dashed]    (498,160) -- (541.25,160.13) ;
% \draw [shift={(543.25,160.13)}, rotate = 180.17] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3706975149666767] 
\draw    (468,160) -- (511.25,160.13) ;
\draw [shift={(513.25,160.13)}, rotate = 180.17] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
% %Shape: Circle [id:dp9882621263515663] 
% \draw[very thick,black]   (448,160) .. controls (448,146.19) and (459.19,135) .. (473,135) .. controls (486.81,135) and (498,146.19) .. (498,160) .. controls (498,173.81) and (486.81,185) .. (473,185) .. controls (459.19,185) and (448,173.81) .. (448,160) -- cycle ;
%Shape: Circle [id:dp9882621263515663] 
\draw[very thick,black]   (418,160) .. controls (418,146.19) and (429.19,135) .. (443,135) .. controls (456.81,135) and (468,146.19) .. (468,160) .. controls (468,173.81) and (456.81,185) .. (443,185) .. controls (429.19,185) and (418,173.81) .. (418,160) -- cycle ;
%Shape: Circle [id:dp7407174319355243] 
\draw   (80.65,178.57) .. controls (80.64,176.6) and (82.22,175) .. (84.19,175) .. controls (86.16,175) and (87.77,176.6) .. (87.79,178.57) .. controls (87.81,180.54) and (86.23,182.13) .. (84.26,182.13) .. controls (82.29,182.13) and (80.67,180.54) .. (80.65,178.57) -- cycle ;
%Shape: Circle [id:dp41729943435639916] 
\draw   (80.65,194.57) .. controls (80.64,192.6) and (82.22,191) .. (84.19,191) .. controls (86.16,191) and (87.77,192.6) .. (87.79,194.57) .. controls (87.81,196.54) and (86.23,198.13) .. (84.26,198.13) .. controls (82.29,198.13) and (80.67,196.54) .. (80.65,194.57) -- cycle ;
%Shape: Circle [id:dp478255207950242] 
\draw   (80.65,209.57) .. controls (80.64,207.6) and (82.22,206) .. (84.19,206) .. controls (86.16,206) and (87.77,207.6) .. (87.79,209.57) .. controls (87.81,211.54) and (86.23,213.13) .. (84.26,213.13) .. controls (82.29,213.13) and (80.67,211.54) .. (80.65,209.57) -- cycle ;

% Text Node
\draw (55,146.4) node [anchor=north west][inner sep=0.75pt]    {$A_{2}( t)$};
% Text Node
\draw (52,220.4) node [anchor=north west][inner sep=0.75pt]    {$A_{N}( t)$};
% Text Node
\draw (55,76.4) node [anchor=north west][inner sep=0.75pt]    {$A_{1}( t)$};
% Text Node
\draw (425,105.4) node [anchor=north west][inner sep=0.75pt]    {$Geo^{[ X]} /D/1$};
%\draw (428,112.4) node [anchor=north west][inner sep=0.75pt]    {$Geo^{[ X]} /D/1$};

\end{tikzpicture}
